Privacy-preserving Chunk Scheduling in a BitTorrent Implementation of Federated Learning

Traditional federated learning (FL) relies on a central aggregator server, which can create performance bottlenecks and privacy risks. Decentralized mix-and-forward designs remove the server, but repeated local mixing can attenuate global information under heterogeneity and expose peer-to-peer neighborhoods as a privacy attack surface. To preserve FedAvg-style aggregation semantics over updates reconstructable by the round deadline while scaling dissemination, we present FLTorrent, a BitTorrent-based dissemination layer for serverless FL with a short warm-up. Warm-up hardens within-round source unlinkability, a dissemination-layer goal orthogonal to content protections such as DP or secure aggregation, via pre-round obfuscation, randomized lags, and coordination-only non-owner-first scheduling with the tracker off the data path, before switching to vanilla BitTorrent swarming. We upper-bound the per-transfer attribution posterior by the fraction of owner chunks in a sender's eligible cover set, and derive a tighter high-probability bound that improves with early non-owner mass. A simple heuristic, GreedyFastestFirst, attains about 92% of a bandwidth-optimal max-flow upper bound, while warm-up remains a stable about 12% share of a round across 100-500 peers. Under an observation-only local adversary, FLTorrent drives attribution success close to neighborhood-level random guessing for typical nodes, improves with network size, and remains robust under collusion. In LLM-scale dissemination stress tests over 7-10 Gbps access links, FLTorrent adds only about 6-10% round-time overhead relative to BitTorrent-only. Overall, FLTorrent shows that within-round unlinkability and BitTorrent-level efficiency can co-exist with predictable, low overheads at scale.

==> Sections/6experiment_backup.tex <==
\section{Performance Evaluation}


% \subsection{ Experimental Results}
This section presents an evaluation of \emph{FLTorrent}, delineating: (1) the bandwidth efficiency of the different centralized heuristics against the max-flow bandwidth optimal solution; (2) the scalability of centralized scheduling compared to the fully distributed one; (3) \emph{FLTorrent}'s robustness in mitigating privacy leakage; (4) the time overhead introduced by \emph{FLTorrent}'s initial warm-up phase in completing a training round vs. the duration of a training round under pure BitTorrent, for different types of ML models and network sizes. We use a random network topology, where nodes exhibit varying neighbor counts above a minimum connection threshold, $min-connection$, and unique uplink/downlink bandwidths, evaluating \emph{FLTorrent}'s robustness in diverse bandwidth scenarios.
To assess the efficacy of our proposed system, we have established several key performance metrics, which are instrumental in quantitatively evaluating the performance of \emph{FLTorrent}. 
\\\textbf{Bandwidth Utilization}: The average bandwidth consumed by peers during the warm-up phase.
\\\textbf{k-Chunk Achievement Ratio}: the ratio of peers that have acquired at least $k$ chunks within a specified time frame.
\\\textbf{Warm-Up Duration}: The time taken from the start of an FL round $t_0$ until all peers possess at least $k$ chunks, $T_{BT}$, marking the transition to normal BitTorrent operations.
\\\textbf{Round Duration}: Total Time of FL round, including warm-up, BitTorrent, and aggregation phases.
\\\textbf{Attack Success Rate (ASR)}: Probability that an attacker identifies the origin of received chunks.
%--------------------------------------------------------------------------------------------------------
\subsection{Setting}
In the initial phase of our simulation setup, \emph{FLTorrent} is calibrated with real-world parameters, utilizing a GoogleNet model size of 51.1 MB ~\cite{shu2018if} and bandwidth reflective of European residential broadband, with uplink speeds of 15.5 to 25.3 Mbps and downlink speeds of 36.5 to 121 Mbps \cite{OECD2024}. The model is divided into 206 chunks of 256KB each, aligning uplink/downlink capacities to [7, 12] and [18, 60] chunks. In our network configuration, we have $n=50$ nodes, with each node maintaining a  $min-connections=5$ nodes. The parameter $R$ is set to represent 20\% of the chunks per gradient. Since each gradient is divided into 206 chunks, 20\% corresponds to $206 \times 0.2 = 41.2 \approx 41$ chunks.The time variable $T$ spans from 0 to 2 seconds, while $k$ remains fixed at 10\% of the total chunk count, i.e., $206 \times 50 = 10300$, which corresponds to $1030$ chunks.

\subsection{FLTorrent vs Gossip DFL vs CFL}
\begin{table}[h]
\centering
\caption{Test Accuracy Comparison of Different Federated Learning Approaches}
\label{tab:accuracy}
\small
\begin{tabular}{llccc}
\toprule
\textbf{Dataset} & \textbf{Data Distribution} & \textbf{CFL} & \textbf{GossipDFL} & \textbf{FLTorrent} \\
\midrule
\multirow{4}{*}{CIFAR-10} 
    & Dirichlet ($\alpha$=0.1) & 0.6883 & 0.3794 & 0.6205 \\
    & Dirichlet ($\alpha$=0.5) & 0.7440 & 0.6329 & 0.6706 \\
    & Dirichlet ($\alpha$=1.0) & 0.7627 & 0.7091 & 0.7218 \\
    & IID                       & 0.8276 & 0.7339 & 0.7913 \\
\midrule
\multirow{4}{*}{MNIST}
    & Dirichlet ($\alpha$=0.1) & 0.9853 & 0.9073 & 0.9784 \\
    & Dirichlet ($\alpha$=0.5) & 0.9929 & 0.9645 & 0.9879 \\
    & Dirichlet ($\alpha$=1.0) & 0.9935 & 0.9720 & 0.9899 \\
    & IID                       & 0.9932 & 0.9861 & 0.9924 \\
\bottomrule
\end{tabular}
\end{table}
50 rounds

\begin{figure*}[t]
\centering

\input{tex/acc}

\caption{}
\label{fig:fl_accuracy_comparison}
\end{figure*}

\subsection{Scalability}

\begin{figure}[h]
    \centering
    \input{tex/scale_warmup}
    \caption{Warm-up duration increases linearly with the number of peers in the system.}
    \label{fig:warmup_duration}
\end{figure}

\begin{figure}[t]
    \centering
    \input{tex/scale_asr}
    \caption{Attack success rates for different inference methods increase with network size.}
    \label{fig:asr_comparison}
\end{figure}

\subsection{k analyses}
\begin{figure}[h]
    \centering
    \input{tex/k_warmup}
    \caption{Warm-up duration and its ratio to total simulation time for different values of $K$.}
    \label{fig:k_sweep_dual}
\end{figure}

\subsection{privacy ablation}

\begin{figure}[h]
    \centering
    \input{tex/privacy_ablation}
    \caption{Normalized warm-up duration relative to baseline. K-anonymity (red bars) adds ~20\% overhead.}
    \label{fig:normalized_warmup_fixed}
\end{figure}

\begin{figure}[h]
    \centering
    \input{tex/privacy_ablation_asr}
    \caption{Normalized warm-up duration relative to baseline. K-anonymity (red bars) adds ~20\% overhead.}
    \label{fig:normalized_warmup_fixed}
\end{figure}

\subsection{attack}

\begin{figure}[h]
    \centering
    \input{tex/k_asr}
    \caption{Minimal impact of K on attack success rate. ASR remains nearly constant ($\approx$11.3\%) across different K values.}
    \label{fig:k_asr_minimal}
\end{figure}

\begin{figure}[h]
    \centering
    \input{tex/min_connection_asr}
    \caption{Attack success rate decreases exponentially with minimum connections. ASR drops below 10\% when $m \geq 15$.}
    \label{fig:min_conn_asr}
\end{figure}

\begin{figure}[h]
    \centering
    \input{tex/attacker_asr}
    \caption{Attack success rate decreases exponentially with minimum connections. ASR drops below 10\% when $m \geq 15$.}
    \label{fig:min_conn_asr}
\end{figure}

\subsection{Bandwidth Utilization and k-Chunk Achievement Ratio}
\begin{figure}[h]
    \centering
    \input{tex/bandwidth_timeslots_seconds.tex}
    \caption{Bandwidth Utilization of Max-flow and Heuristics Across Transmission Stages and Warm-Up Duration}
    \label{fig:bandwidth}
\end{figure}
Figure~\ref{fig:bandwidth}a and ~\ref{fig:bandwidth}b present a comparative analysis of bandwidth utilization for different centralized scheduling methods, delineated across chunk transmission stages and time in seconds. Due to bandwidth constraints, only a limited number of chunks can be distributed per unit of time, necessitating multiple reschedules. A transmission stage is defined as the number of scheduling steps in which all nodes can theoretically finish transmitting all missed chunks until they achieve at least $k$ chunks. Figure~\ref{fig:bandwidth}a demonstrates the superior bandwidth utilization of the max-flow over heuristics, completing scheduling within 56 stages for a DL round. In contrast, the most efficient centralized heuristic, GreedyFastestFirst, finishes its process at 135 stages. Transmission stages are ideally completed within 1s, yet scheduler overhead extends this duration. By enhancing the tracker's capabilities, it can reduce these delays and achieve faster completion times.



% \begin{figure}[t]
%     \centering
%     % Subfigure 1
%     \begin{subfigure}{.48\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/bandwidth_timeslots.png}
%         \caption{Bandwidth Utilization vs. Transmission Stages} % Caption for the first subfigure
%          \label{fig:Band_tS}
        
%     \end{subfigure}
%     \hfill % You may adjust or remove this space
%     % Subfigure 2
%     \begin{subfigure}{.48\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/bandwidth_seconds.png}
%         \caption{Bandwidth Utilization vs. Time} % Caption for the second subfigure
%          \label{fig:Band_time}
        
%     \end{subfigure}
    
%     \caption{Bandwidth Utilization of Max-flow and Heuristic Scheduling Methods Across Transmission Stages and Time}
%     \label{fig:bandwidth}
% \end{figure}
 While max-flow exhibits superior bandwidth utilization, leading to fewer transmission stages, its complexity in execution time for practical purposes impedes its practical feasibility. Figure~\ref{fig:bandwidth}b depicts the bandwidth utilization of various centralized scheduling methods over wall-clock time in seconds, indicating the trade-off between max-flow's bandwidth optimization and its operational demands. Max-flow's Warm-Up Duration of about 8000s starkly contrasts with GreedyFastestFirst's 675s, highlighting a significant gap in performance between heuristic methods and max-flow. The superior performance of max-flow in transmission stages, compared to its poorer showing in seconds, results from its bandwidth optimization within each stage and lower time efficiency. While max-flow's bandwidth optimization transmits all required chunks in fewer stages, its extended computation time increases each stage's duration and delays subsequent transmissions, as each must wait for the completion of its scheduling. Consequently, the near-optimal bandwidth utilization and low warm-up duration of different heuristics justify their adoption for \emph{FLTorrent} chunk scheduling in decentralized settings. Among these, the GreedyFastestFirst strategy emerges as the most efficient, demonstrating superior bandwidth utilization and shorter warm-up duration.
%\subsection{Comparative Analysis of GreedyFastestFirst}

% \begin{figure}[t]
%     \centering
%     \input{tex/P_chunks_second.tex}
%     \caption{P-Chunk Achievement Ratio Over Time}
%     \label{fig:p_s}
% \end{figure}

Figure~\ref{fig:bandwidth}c illustrates the progression of $k$-chunk achievement ratio over time using centralized heuristic methods. Due to the excessively high warm-up duration with max-flow, it has been excluded from these comparisons. The findings highlight the superior performance of the GreedyFastestFirst algorithm compared to other heuristics, with GreedyFastestFirst reaching $k$-anonymity at approximately 675.97s, compared to around 1400s for other heuristics. This is attributed to its superior bandwidth utilization in each transmission stage, as depicted in Figure~\ref{fig:bandwidth}a.



% \begin{figure}
%     \centering
%     \includegraphics[scale=0.21]{figures/P_chunks_second.png}
%     \caption{Progression of Nodes Achieving At Least P-Chunks Over Time for Different Heuristic Methods}
%     \label{fig:p_s}
% \end{figure}



% Figure~\ref{fig:s_N} illustrates the scalability of the GreedyFastestFirst heuristic as the network size ranges from 40 to 100 nodes, with $min-connections$ varying from 5 to 25 nodes. While increasing the number of nodes in the network raises the execution time of heuristics, Greedy-FastestFirs demonstrates a less pronounced increase compared to other methods, indicating its stable scalability within an expanding network. For instance, the execution time gap between GreedyFastestFirst and RandomFastestFast is 13.7\% for 50 nodes, whereas it expands to 15.6\% for 100 nodes, highlighting GreedyFastestFirst's relative robustness and accentuating the potential scaling limitations of alternative heuristic approaches. Similarly, the analysis of heuristic execution times concerning varying $min-connections$ suggests that GreedyFastestFirst's execution time does not linearly increase as the number of neighbors of a peer increases, indicating sustained efficiency regardless of network connectivity. 
% \begin{figure}[t]
%     \centering
%     % Subfigure 1
%     \begin{subfigure}{.45\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/plots_network_peerchanges.png}
%         \caption{Execution time vs.  number of peers} % Caption for the first subfigure
%         % \label{fig:Band_tS}
        
%     \end{subfigure}
%     \hfill % You may adjust or remove this space
%     % Subfigure 2
%     \begin{subfigure}{.49\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/plots_network_minconnection_changes.png}
%         \caption{Execution time vs. min-connections} % Caption for the second subfigure
%          % \label{fig:Band_time}
        
%     \end{subfigure}
    
%     \caption{Execution Time Analysis of GreedyFastestFirst Under Variable Network Sizes and Connectivity}
%     \label{fig:s_N}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\linewidth]{figures/plots_network_timechange.png}
%     \caption{Execution Time Analysis of GreedyFastestFirst Under Variable Network Sizes and Connectivity}
%     \label{fig:s_N}
% \end{figure}

% \begin{figure*}[t]
%     \centering
%     % Subfigure 1
%     \begin{subfigure}[t]{.25\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/Distributed_Scheduling_stage_changes.png}
%         \caption{Bandwidth Utilization vs. Transmission Stages} % Caption for the first subfigure
%         \label{fig:Dis_BW_ts}
%     \end{subfigure}%
%     \hfill
%     % Subfigure 2
%     \begin{subfigure}[t]{.25\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/Distributed_Scheduling_second_changes.png}
%         \caption{Bandwidth Utilization vs. Time} % Caption for the second subfigure
%          \label{fig:Dis_BW_se}
%     \end{subfigure}%
%     \hfill
%     % Subfigure 3
%     \begin{subfigure}[t]{.25\linewidth}
%         \centering
%     \includegraphics[height=3.20cm, width=\linewidth]{figures/Distributed_Scheduling_Time.png}
%     \caption{Execution Time vs. Network Sizes}
%     \label{fig:Dis_time}
%     \end{subfigure}
%     \caption{Bandwidth Utilization and Execution Time Comparison of Distributed Scheduling and Centralized GreedyFastestFast}
%     \label{fig:distributed_plot}
% \end{figure*}

% \subsection{Comparing Centralized and Distributed Heuristics}
% The heuristic scheduling methods, while effective in managing chunk transmission among peers, are centrally managed by a tracker, which can introduce significant overhead and limit scalability. This section evaluates the efficiency of \emph{FLTorrent}'s centralized scheduling against distributed scheduling to discern the optimal scenarios for selecting between centralized and distributed approaches.

% \begin{figure}[h]
%     \centering
%     \input{tex/Distributed_Scheduling_BW}
%     \caption{Bandwidth Utilization and Warm-Up Duration of Distributed Scheduling and GreedyFastestFirst}
%     \label{fig:distributed_plot}
% \end{figure}


% Figure~\ref{fig:distributed_plot} contrasts the bandwidth utilization and warm-up duration of GreedyFastestFirst and distributed scheduling with $n$ set to 50 for this experiment, where we assumed the tracker has the same processing resources as other peers. Figure ~\ref{fig:distributed_plot}a demonstrates the GreedyFastestFirst algorithm's optimal bandwidth utilization among peers in the early stages, which leads to a swift completion of the warm-up phase. This efficiency stems from the tracker's detailed awareness of the chunks held by each peer and their bandwidth capacities, allowing for optimized centralized scheduling for peak bandwidth utilization. GreedyFastestFirst finalizes scheduling in just 138 stages, in stark contrast to distributed scheduling's 174 stages. 
% Figure~\ref{fig:distributed_plot}b indicates that the centralized GreedyFastestFirst approach completes its scheduling in just 675s, whereas the distributed method takes considerably longer, finishing in 1478s, representing an improvement percentage of approximately 54\%. This substantial gap in warm-up duration, more pronounced than in transmission stages, emphasizes the benefits of having a centralized tracker. With detailed insight into each peer's bandwidth, the tracker makes informed decisions to optimize bandwidth use early, shortening the warm-up phase.
% % \begin{figure}
% %     \centering
% %     \includegraphics[width=0.5\linewidth]{figures/Distributed_Scheduling_Time.png}
% %     \caption{Execution Time Comparison of GreedyFastestFirst and Distributed Scheduling Under Variable Network Sizes}
% %     \label{fig:Dis_time}
% % \end{figure}

% Although results of Figures~\ref{fig:distributed_plot}a and ~\ref{fig:distributed_plot}b with $n=50$ peers indicate better bandwidth utilization and shorter warm-up phase in centralized scheduling, warm-up duration differences varying on network size due to changes in task complexity for both centralized and distributed scheduling. Figure~\ref{fig:distributed_plot}c showcases the impact of network scale on the warm-up duration for centralized and distributed scheduling algorithms. The result reveals that as the number of peers increases, the gap between centralized and distributed scheduling narrows. For networks with fewer than 85 peers, centralized scheduling shows better warm-up duration due to optimized bandwidth utilization. However, beyond 85 peers, centralized scheduling incurs longer warm-up duration due to increased tracker processing workload. Distributed scheduling becomes more efficient as the network grows, spreading the processing workload across nodes. It's worth noting that our experiment assumed the tracker has the same processing resources as other peers. In scenarios where the tracker has greater capacities, centralized scheduling could be more efficient, potentially increasing the threshold for distributed scheduling to become superior over centralized scheduling.  
% %////////////////////////////////
% % \begin{figure}[t]
% %     \centering
% %     % Subfigure 1
% %     \begin{subfigure}{.49\linewidth}
% %         \centering
% %         \includegraphics[width=\linewidth]{figures/plots_attack_peer_changes.png}
% %         \caption{ASR based on varying number of peers} % Caption for the first subfigure
% %         % \label{fig:Band_tS}
% %      \label{fig:privacy_FL_peers}    
% %     \end{subfigure}
% %     \hfill % You may adjust or remove this space
% %     % Subfigure 2
% %     \begin{subfigure}{.49\linewidth}
% %         \centering
% %         \includegraphics[width=\linewidth]{figures/plots_attack_connection_changes.png}
% %         \caption{ASR based on varying min-connections} % Caption for the second subfigure
% %          % \label{fig:Band_time}
% %         \label{fig:privacy_FL_connections}
% %     \end{subfigure}
    
% %     \caption{Attack success rate of \emph{FLTorrent} Under Variable Network Sizes and connectivity}
% %     \label{fig:privacy_FL}
% % \end{figure}



% \subsection{Privacy Analysis}\label{sec:upperbound}

% \begin{figure}[h]
%     \centering
%     \input{tex/plots_attack_connection_peers.tex}
%     \caption{ASR vs. Network Sizes and Connectivity}
%     \label{fig:privacy_FL}
% \end{figure}

In this section, we assess the success of attacks against various topologies and \emph{FLTorrent}'s role in reducing their average ASR. Figure~\ref{fig:privacy_FL}a and Figure~\ref{fig:privacy_FL}b present the ASR of three distinct attacks relative to the number of peers and $min-connections$ respectively. The \emph{Ideal} line in Figure~\ref{fig:privacy_FL}a and b models an optimal state of privacy, where the origins of data chunks are completely obscured, while the \emph{Upperbound} line illustrates the maximum ASR (see Sec.~\ref{sec:probability}: $x=0, R=0$). In this study, centralized GreedyFastestFirst was selected for task scheduling based on its proven superior performance. Figure~\ref{fig:privacy_FL}a demonstrates a clear reduction in \emph{FLTorrent} ASR with an increase in peer count. Specifically, the ASR for clustering, amount greedy, and sequential greedy strategies decreases from 16.0\%, 16.0\%, and 14.0\% at $n=10$, which is closer to the ideal rather than the upper bound, to 2.36\%, 2.36\% and 2.88\% at $n=50$, respectively, matching the ideal value. This observation aligns with our probabilistic analysis, showing that the ASR decreases as the network grows, since peers disseminate chunks within larger groups, promoting chunk diffusion across the network. This trend towards the \emph{Ideal}, along with the widening gap from the \emph{Upperbound}, highlights \emph{FLTorrent}'s effective privacy safeguards. 



The analysis of ASR based on $min-connections$ in ~\ref{fig:privacy_FL}b reveals that increasing the $min-connections$ leads to a notable rise in the \textit{Upperbound}, suggesting that more connections per node complicate accurate source attribution of a chunk, potentially heightening ASR. Despite this, \emph{FLTorrent}'s ASR remains below 10\% and comparable to \textit{Ideal} for various attack strategies. This effectiveness ensures that ASR in \emph{FLTorrent} remains close to the \emph{Ideal} and away from the \textit{Upperbound}.

% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\linewidth]{figures/plots_attack_connection_peers.png}
%     \caption{Attack success rate of \emph{FLTorrent} Under Variable Network Sizes and connectivity}
%     \label{fig:a_c_p}
% \end{figure}
%///////////////////
% \begin{figure}[t]
%     \centering
%     % Subfigure 1
%     \begin{subfigure}{.49\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/pre_round_compare_peer_changes.png}
%         \caption{ASR based on varying number of peers} % Caption for the first subfigure
%         \label{fig:Privacy_increase_peer}
        
%     \end{subfigure}
%     \hfill % You may adjust or remove this space
%     % Subfigure 2
%     \begin{subfigure}{.49\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/pre_round_compare_connection_changes.png}
%         \caption{ASR based on varying min-connections} % Caption for the second subfigure
%          \label{fig:Privacy_increase_connection}
        
%     \end{subfigure}
    
%     \caption{ASR of clustering attack based on applying different levels of privacy-preserving mechanisms}
%     \label{fig:Privacy_increase}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \input{tex/pre_round_compare.tex}
%     \caption{ASR of clustering attack based on applying different levels of privacy-preserving mechanisms}
%     \label{fig:ASR_incremental}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/pre_round_compare.png}
%     \caption{Attack success rate of clustering attack based on applying different levels of privacy-preserving mechanisms}
%     \label{fig:i_a_p}
% \end{figure}
We also conducted a more in-depth ``incremental'' analysis to evaluate the impact of the different privacy preservation layers in \emph{FLTorrent}. Figure~\ref{fig:privacy_FL}c and ~\ref{fig:privacy_FL}d present the ASR of the clustering attack strategy under various combinations of obfuscation mechanisms, including pre-round obfuscation and random delays based on varying numbers of peers and $min-connections$. The clustering attack strategy was employed in our analysis due to its slight superiority to the greedy algorithm, both of which are recognized as the attack methods with the highest ASR in our context. Notably, both the value of $R$ for pre-round obfuscation and $T$  for time obfuscation were kept minimal to prevent excessive system overhead.  The findings of Figure~\ref{fig:privacy_FL}c and ~\ref{fig:privacy_FL}d reveal that the combination of both, \textit{pre-round obfuscation+  random lags} results in the lowest ASR 2.36\% compared with \textit{No pre-round obfuscation and random lags}, \textit{only random lags}, and \textit{only pre-round obfuscation} by the average of 4.6\%, 4.0\% and 4.4\% respectively. Without these measures, ASR is highest, but implementing both improves privacy before transitioning to standard BitTorrent. As demonstrated in earlier probabilistic analysis, increasing peers or reducing neighbor connections lowers the chance of receiving a chunk from the sender's original set. The findings align with probabilistic results, where fewer peer-to-peer links decrease the likelihood of information leakage, reducing ASR.
\subsection{Evaluating the Impact of Privacy Mechanisms on FL Round Duration for LLMs}
 To assess the impact of incorporating privacy-preserving considerations into BitTorrent chunk scheduling on the duration of Fl rounds in \emph{FLTorrent}'s, we compared it against standard BitTorrent over a full training round. Figure ~\ref{fig:time_llm} displays the round duration and its normalized values of different schedulers deployed for running LLMs. This evaluation utilized four major LLMs: Google's Gemma-7B \cite{GEMMA7B}, with a size of 17.7 GB, part of a suite built on the same research as the Gemini models; NVIDIA's Chat with RTX\cite{RTX}, sized 35.1 GB; EleutherAI's open-source GPT-J\cite{GPT-J}, which is 61.1 GB in size; and the strongest open-source Smaug-72B-v0.1\cite{Smaug}, with a size of 144.58 GB. For this analysis, the bandwidth range for uplink/downlink is set between 7 to 10 Gbps.
% \begin{figure}
%     \centering
%     % Subfigure 1
%     \begin{subfigure}{.49\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/seconds for big models.png}
%         % Adjust the width as necessary to fit
%     \end{subfigure}
%     \hfill % You may adjust or remove this space
%     % Subfigure 2
%     \begin{subfigure}{.49\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/normalized seconds for big models.png}
%         % Adjust the width as necessary to fit
%     \end{subfigure}
    
%     \caption{Round Duration and Normalized Values Across Schedulers for LLMs}
%     \label{fig:time_llm}
% \end{figure}

\begin{figure}[h]
    \centering
    \input{tex/llm_time}
    \caption{Round Duration and Normalized Values Across Schedulers for LLMs}
    \label{fig:time_llm}
\end{figure}

Based on Figure \ref{fig:time_llm}, \emph{FLTorrent} slightly increases round duration due to its privacy-preserving layer establishing $k$-anonymity before transitioning to BitTorrent. Although this additional step increases the number of peer-to-peer and peer-to-tracker communications in \emph{FLTorrent} compared to BitTorrent, crucial for obscuring the origins of the received chunks, significantly mitigating the ASR. Specifically, \emph{FLTorrent} accounts for an increase in round duration of 36.88\%, 6.6\%, 7.1\%, and 11.66\% for Gemma-7B, Chat with RTX, GPT-J, and Smaug-72B-v0.1, respectively. Despite this overhead, as demonstrated in Figure \ref{fig:privacy_FL}, the integration of privacy-preserving mechanisms decreases the ASR to a maximum of 18\%. The overhead introduced by \emph{FLTorrent} is vindicated by the pronounced decrement in ASR, indicating its privacy-preserving efficacy within distributed learning networks.

==> Sections/Background.tex <==
\section{Background}
\subsection{FL and DL}
% -- two paragraphs
FL enables $n$ clients (nodes) to train a global model $\weights$ collaboratively without revealing their local datasets. Unlike centralized learning, where local datasets have to be collected by a central server before training, FL requires clients to upload the weights of local models ($\{\weights^v \mid v \in n\}$) to a parametric server. 
Specifically, FL aims to optimize a loss function: $\mathop {\min }\limits_\weights \ \ell (\weights ) = \sum\limits_{v = 1}^n {\frac{{{|D_v|}}}{D}{L_v}(} \weights ),{L_v}(\weights ) = \frac{1}{{{|D_v|}}}\sum\limits_{j \in {D_v}} {{\ell _j}(\weights, x_j)}$, where ${L_v}(\weights )$ and $|D_v|$ are the loss function and local data size of client $v$, respectively. $D_v$ refers to the set of data indices with size $|D_v|$. Additionally, $D$ is the total size of the global dataset. Without loss of generality and correctness, at the $t$-th iteration, the training of FL can be divided into 3 main steps: \\
%\begin{itemize}
1) \textit{Global model download}. The server selects partial clients engaging in training. All connected clients download the global model $\weights_t$ from the server.\\
2) \textit{Local training}.  Each client updates its model by training with it's own dataset: $\weights_t^v \leftarrow \weights_t^v-\eta\frac{\partial L(\weights_t, b)}{\partial \weights_t^v} $, where $\eta$ and $b$ refer to learning rate and local batch, respectively. \\
3) \textit{Aggregation}. After the clients upload their local updates $\{\weights^v_t \mid v \in n\}$, the server can output the new global model via Federated Averaging (FedAvg): $\weights_{t+1} \leftarrow \sum\limits_{i = 1}^n \frac{{{|D_i|}}}{D} \weights_t^v.$

Decentralized Learning (DL) represents a paradigm shift in distributed machine learning methodologies, distinguishing itself from FL by eliminating the reliance on an aggregator. In this approach, each client actively engages in a P2P model, fostering a decentralized network where nodes communicate directly with one another. During each iteration, followed by steps 1 and 2 of FL, clients receive model updates from their neighbors, and mix them locally:
$\weights_{t+1} \leftarrow \sum\limits_{\node \in \neighborhood(\node)} \frac{{{|D_v|}}}{D} \weights_t^v,$
where $\neighborhood(\node)$ stands for the neighbors of client $v$.
After that, they forward the aggregated updates to their neighboring clients. Figure~\ref{fig:flvsdl} shows the differences between FL and DL. In FL, all clients equally contribute to a shared global model, whereas in DL, local models primarily influence their combined models.
\subsection{The BitTorrent Protocol}

The BitTorrent protocol~\cite{cohen2003incentives}, a popular peer-to-peer (P2P) file-sharing system, operates by distributing files into small chunks across a network of nodes, or peers. These peers exchange chunks in parallel, enhancing download and upload speeds. Central to this system is the tracker, a server that coordinates initial peer connections but does not track the specific chunks each peer holds. Additionally, BitTorrent utilizes a "choke/unchoke" mechanism, which selectively restricts or allows data flow to peers based on their reciprocation rate. This strategy prioritizes peers who have recently shared data at high rates, optimizing bandwidth use. The protocol enables simultaneous downloads from multiple peers, thereby improving data distribution's efficiency, speed, and reliability.  Additionally, it is resilient to free-riders, ensuring robust data sharing even if some peers do not upload chunks. 

% The BitTorrent protocol~\cite{cohen2003incentives}, a widely adopted P2P file-sharing mechanism, operates on a robust foundation of distributed data exchange. In this decentralized ecosystem, files are divided into smaller chunks and distributed across a network of interconnected nodes, known as peers. Peers collaboratively share these chunks with the neighbors, allowing for parallel downloading and uploading. At the heart of this system is the tracker, a central server that facilitates the initial communication between peers. The tracker merely records the participation of peers in a specific torrent without maintaining knowledge of the individual data chunks each peer possesses. Additionally, BitTorrent employs a so-called \textit{choke/unchoke} mechanism that ``chokes'', i.e., avoids sending chunks to peers that don't reciprocate by sending chunks back at a high rate, whereas it ``unchokes'', i.e., honors requests to send missing chunks to peers that in the recent past have reciprocated by sending chunks back at a high rate.  What distinguishes BitTorrent is its efficient  bandwidth utilization, as peers can simultaneously download chunks from multiple peers, optimizing data distribution and enhancing the speed and reliability of data retrieval and it's resilience to free-riding peers that do not contribute to the group by uploading chunks to others. 

%\subsection{Privacy Attacks on FL and DL}
% As previously mentioned, to maintain compatibility with existing poisoning attack defenses, we retained node pseudo-identities (pseudo-identity) and data chunk identifiers (chunk ID) to enable reputation-based defense mechanisms. However, this significantly increases the risk of identity correlation attacks at the BitTorrent layer. Specifically, during the early stages of a training round, nodes typically only possess local gradient chunks. As a result, a malicious node could infer that these early transmitted chunks likely belong to the sender and, by analyzing the gradient information within these chunks, successfully match the node's identity with its private data.Due to the presence of explicit identity and data markers, traditional FL privacy defense mechanisms, such as differential privacy and secure multiparty computation (SMPC)~\cite{truex2019hybrid,bonawitz2017practical}, offer limited protection against such attacks.
%\subsection{System and Threat Model}
%This section formalises the operational assumptions of FLTorrent and delineates the class of adversaries we defend against. 




% \NL{1-2 citations}
% Typically, the workflow of MIA is as follows:\\
% 1) The adversary collects publicly available data that is similar or representative of the target model's training data.\\
% 2) The adversary trains multiple shadow models on the collected data. Each shadow model is designed to mimic the behavior of the target model as closely as possible.\\
% 3) The shadow models are labeled with the predictions made on the training data. Then the adversary selects a shadow model that performs well on the training data and is considered a good approximation of the target model.\\
% 4) The adversary creates a set of data points and wants to determine their membership in the target model's training dataset. The adversary feeds the attack data points to both the target model and the selected shadow model.
% By comparing the outputs and behaviors of the two models, the adversary tries to infer whether a specific data point was part of the target model's training dataset. 
% \LNC{These attacks are not directly protected in our protocols for now, so maybe we shouldn't mention them? Our protocol currently only protects gradients and pairwise relationships between nodes’ id. Or we can emphasize that in our protocol, even if an attacker obtains some private information from a gradient, the inability to correspond this private information to a specific node protects privacy to some extent.}
% \NL{I agree with Neicheng's comment. Just put few references to these attacks but do not describe them in order to save space. Then at the end say that these attacks are orthogonal to what we do, which is to protect the BitTorrent protocol that we use from timing attacks at the begining of the round targeting on revealing the association between peer and chunk ids.}

==> Sections/notation.tex <==
\subsection{Notation}
\label{sec:notation}

The frequently used notations are summarized in Table~\ref{tab:notations}.
\begin{table}[t]
\centering
\begin{tabular}{@{}c|l@{}}
\toprule
 \textbf{Notation}&  \textbf{Description}  \\ \midrule
 $\node$ & Node \\
 $\gradient$ & Gradient \\
 $t$ & Time \\
 $\upbandwidth(\node)$ & Uplink bandwidth of node $\node$\\
 $\downbandwidth(\node)$ & Downlink bandwidth of node $\node$ \\
 $\setofnodes$ & A set of nodes \\ 
 $\neighborhood(\node)$ & The neighborhood of node $\node$  \\ 
 $\setofchunks(\cdot)$ & A set of chunks \\  
 $\setofgradients(\cdot)$ & A set of gradients  \\  
 $\announce$ & Announcement \\
 $\gannounce$ & Neighborhood-wide announcements \\
 $\completiontime(\cdot)$ & Completion time\\
 $\avgbandwidth$ & Average bandwidth \\
 $\ppmodel$ & P2P model \\
 
 \bottomrule
\end{tabular}
\caption{Notation summary}
\label{tab:notations}
\end{table}
